A flexible FPGA accelerator for convolutional neural networks

Though CNNs are highly parallel workloads, in the absence of efficient on-chip memory reuse techniques, an accelerator for them quickly becomes memory bound. In this paper, we propose a CNN accelerator design for inference that is able to exploit all forms of reuse available to minimize off-chip memory access while increasing utilization of available resources. The proposed design is composed of cores, each of which contains a one-dimensional array of processing elements. These cores can exploit different types of reuse available in CNN layers of varying shapes without requiring any reconfiguration; in particular, our design minimizes underutilization due to problem sizes that are not perfect multiples of the underlying hardware array dimensions. A major obstacle in the adoption of FPGAs as a platform for CNN inference is the difficulty to program these devices using hardware description languages. Our end goal is to also address this, and we develop preliminary software support via a codesign in order to leverage the accelerator through TensorFlow, a dominant high-level programming model. Our framework takes care of tiling and scheduling of neural network layers and generates necessary low-level commands to execute the CNN. Experimental evaluation on a real system with a PCI-express based Xilinx VC709 board demonstrates the effectiveness of our approach. As a result of an effective interconnection, the design maintains a high frequency when we scale the number of PEs. The sustained performance overall is a good fraction of the accelerator's theoretical peak performance.

==> Makefile <==
#
# $Id: Makefile,v 1.1.1.1 2011/12/05 09:52:11 uday Exp $
#

LATEX := latex
BIBTEX := bibtex
L2H := latex2html
PDFLATEX := pdflatex
DVIPS := dvips
GOALS := paper.pdf #paper.pdf
SUBDIRS := tikz

all: $(GOALS)


%.pdf: %.tex tex/*.tex tikz/*.tex bibfile.bib code/*.cpp
	make -C tikz/
	latexmk -pdf $<

subdir_clean:
	for dir in $(SUBDIRS); do \
		( cd $$dir; ${MAKE} clean ); \
	done

clean:
	rm -f *.aux *.bak *.log *.blg *.brf *.cb *.ind *.idx *.ilg  \
		*.inx *.ps *.dvi *.pdf *.toc *.out *.bak fig/*.bak \
		*.fdb_latexmk *.fls *.xcp *.gz
	for dir in $(SUBDIRS); do \
		( cd $$dir; ${MAKE} clean ); \
	done


cleaner:
	make --no-print-directory -C tikz cleaner
	-rm -f *.aux *.bak *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg  \
		*.inx *.ps *.dvi *.pdf *.toc *.out *.bak fig/*.bak \
		*.fdb_latexmk *.fls *.xcp *.gz


==> tex/pseudocode1.tex <==



==> tikz/Makefile <==
EPS := tiling.eps fpga_pipeline.eps conv.eps conv2.eps dilation.eps pe.eps table.eps framework.eps
CURRENT := pe.eps


all: $(EPS)

current: $(CURRENT)

PDFS := $(EPS:.eps=.pdf)

pdf: $(PDFS)

%.pdf: %.eps
	epstopdf $<

%.eps: %.tex 
	pdflatex $<
	pdftops -eps $*.pdf

clean:
	rm -f *.aux *.bak *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg  \
		*.inx *.ps *.dvi *.pdf *.toc *.out *.bak fig/*.bak \
		*.fdb_latexmk *.fls *.xcp *.gz

cleaner:
	rm -f *.aux *.bak *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg  \
		*.inx *.ps *.dvi *.pdf *.toc *.out *.bak fig/*.bak \
		*.eps


==> tikz/mlt.tex <==
\usetikzlibrary{shapes,arrows}
\usetikzlibrary{positioning, fit}
\usetikzlibrary{matrix}
\usetikzlibrary{calc}
\usetikzlibrary{decorations.pathreplacing}
% Define box and box title style
\tikzstyle{picnode} = [inner sep=0pt]
\tikzstyle{fancytitle} = [draw, fill=blue!20, rectangle, rounded corners]


\tikzstyle{dullblock} = [draw, fill=black!20, circle, minimum height=2em, minimum width=2em]
\tikzstyle{block} = [draw=black!100, thick, line width=0.2mm, fill=blue!20, rectangle, minimum height=1em, minimum width=1em]
\tikzstyle{blocksmall} = [draw=blue!80, thick, line width=0.2mm, fill=blue!20, rectangle, minimum height=1em, minimum width=1em]
\tikzstyle{group} = [draw=red!100, very thick, rectangle, rounded corners, minimum height=2em, minimum width=2em]
\tikzstyle{textblock} = [draw, fill=blue!20, rectangle, rounded corners]
\tikzstyle{input} = [draw, thick, fill=blue!20, circle, minimum size=1pt]
\tikzstyle{output} = [draw, fill=blue!20, circle, minimum size=1pt]
\tikzstyle{pinstyle} = [pin edge={to-,thin,black}]

\definecolor{forestgreen}{rgb}{0.0, 0.5, 0.0}


\newcommand{\overlaplogo}[0]{
    %\begin{overlayarea}{\textwidth}{\textheight}
    \begin{tikzpicture}[scale=0.8]
        \drawgrid{290pt}{72pt}{}{}{16pt}{36pt}
        %\drawgrid{592pt}{48pt}{}{}{16pt}{24pt}

        \drawiterations{0}{16}{0}{2}{16pt}{24pt}{2pt}{blue!100}
        \drawliveouts{0}{16}{2}{2}{16pt}{24pt}{2pt}{red!100}

        \drawaffinedeps{1}{16}{1}{1}{16pt}{24pt}{1}{0}{0}{1}{-1}{-1}{black!100}
        \drawaffinedeps{0}{16}{2}{2}{16pt}{24pt}{1}{0}{0}{1}{0}{-1}{black!100}

        \drawaffinedeps{0}{16}{1}{1}{16pt}{24pt}{1}{0}{0}{1}{0}{-1}{black!100}
        \drawaffinedeps{0}{15}{1}{1}{16pt}{24pt}{1}{0}{0}{1}{1}{-1}{black!100}
        \drawaffinedeps{0}{14}{2}{2}{16pt}{24pt}{1}{0}{0}{1}{2}{-1}{black!100}

        %\node [x=16pt, y=24pt, anchor=east](f1) at (-1, 0) {\small$f_1$};
        %\node [x=16pt, y=24pt, anchor=east](f2) at (-1, 1) {\small$f_2$};
        %\node [x=16pt, y=24pt, anchor=east](flive) at (-1, 2) 
        %{\small$f_{out}$};
        %\node [x=16pt, y=24pt, anchor=east](flive) at (4, 3.5) {\small P1};
        %\node [x=16pt, y=24pt, anchor=east](flive) at (9, 3.5) {\small P2};
        %\node [x=16pt, y=24pt, anchor=east](flive) at (14, 3.5) {\small P3};
 
        % Draw the tiles
        \filldraw[thick,fill=green!70!black,fill opacity=0.4, x=16pt, y=24pt, rounded corners] (5.5, -0.5) -- (7, 2.5) -- (12.5, 2.5) -- (18.5, -0.5)  -- cycle;
        \filldraw[thick,fill=green!70!black,fill opacity=0.4, x=16pt, y=24pt, rounded corners] (-0.5, -0.5) -- (1, 2.5) -- (5.5, 2.5) -- (11.5, -0.5)  -- cycle;
        \filldraw[thick,fill=blue!90!black,fill opacity=0.3, x=16pt, y=24pt, rounded corners] (12.4, -0.3) -- (7.2, 2.3) -- (9.8, 2.3) -- (15.2, -0.3)  -- cycle;
        \filldraw[thick,fill=blue!90!black,fill opacity=0.3, x=16pt, y=24pt, rounded corners] (15.5, -0.3) -- (10.1, 2.3) -- (12.65, 2.3) -- (17.85, -0.3)  -- cycle;
        %\filldraw[thick,fill=green!90!black,fill opacity=0.2, x=16pt, y=24pt, rounded corners] (9.5, -0.5) -- (3.5, 2.5) -- (6.5, 2.5) -- (12.5, -0.5)  -- cycle;
        %\filldraw[thick,fill=green!90!black,fill opacity=0.2, x=16pt, y=24pt, rounded corners] (7.5, -0.5) -- (1.5, 2.5) -- (4.5, 2.5) -- (10.5, -0.5)  -- cycle;
        
        \drawliveouts{0}{16}{2}{2}{16pt}{24pt}{2pt}{red!100}
    \end{tikzpicture}
    %\end{overlayarea}
}

\newcommand{\drawaffinedeps}[9]{%
    \def\tempa{#1}%
    \def\tempb{#2}%
    \def\tempc{#3}%
    \def\tempd{#4}%
    \def\tempe{#5}%
    \def\tempf{#6}%
    \def\tempg{#7}%
    \def\temph{#8}%
    \def\tempi{#9}%
    \drawaffinedepscontinued
}

\newcommand{\drawaffinedepscontinued}[4]{
% x-start x-end y-start y-end x-gap y-gap a b c d tx ty color arrowgap
% | a b || x | + | tx | = | x' |
% | c d || y |   | ty |   | y' |
% Draws an arrow from (x', y') to (x, y)
\foreach \x in {\tempa,...,\tempb}
    \foreach \y in {\tempc,...,\tempd} {
       \draw [->,>=stealth,>=stealth, color=#4] [x=\tempe, y=\tempf]($ (#2, #3) + \tempg*(\x, 0) + \temph*(\y, 0) + \tempi*(0, \x) + #1*(0, \y) $) -- (\x \y);
    }
}

\newcommand{\drawgrid}[6]{
% x-range y-range x-label y-label x-gap y-gap
\draw[help lines, very thin, dashed] (-#5,-#6) grid [xstep=#5, ystep=#6] (#1, #2);
% axis and lables 
%\draw [<->,thick] (-#5,#2+#6) node (yaxis) [above] {$#4$}
%        |- (#1+#5, -#6) node (xaxis) [right] {$#3$};
}

\newcommand{\drawiterations}[8]{
% x-start x-end y-start y-end x-gap y-gap size
\foreach \x in {#1,...,#2}{
    \foreach \y in {#3,...,#4} {
        \node[circle, draw, fill=#8, x=#5, y=#6, minimum size = 2*#7, inner sep = 0pt] (\x \y) at (\x, \y) {};
        %\fill[color=#8] [x=#5, y=#6](\x, \y) circle(#7);
    }
}
}

\newcommand{\drawliveouts}[8]{
% x-start x-end y-start y-end x-gap y-gap size
\foreach \x in {#1,...,#2}{
    \foreach \y in {#3,...,#4} {
        \node[circle, thick, draw, color=#8, x=#5, y=#6, minimum size = 3*#7, inner sep = 0pt] (\x \y) at (\x, \y) {};
    }
}
}

\newcommand{\drawcircles}[8]{
% x-start x-end y-start y-end x-gap y-gap size
\foreach \x in {#1,...,#2}{
    \foreach \y in {#3,...,#4} {
        \node[circle, draw, color=#8, x=#5, y=#6, minimum size = 2*#7, inner sep = 0pt] (\x \y) at (\x, \y) {};
        %\fill[color=#8] [x=#5, y=#6](\x, \y) circle(#7);
    }
}
}

